Tackling Catastrophic Forgetting and Background Shift in Continual Semantic Segmentation

Deep learning approaches are nowadays ubiquitously used to tackle computer vision tasks such as semantic segmentation, requiring large datasets and substantial computational power. Continual learning for semantic segmentation (CSS) is an emerging trend that consists in updating an old model by sequentially adding new classes. However, continual learning methods are usually prone to catastrophic forgetting. This issue is further aggravated in CSS where, at each step, old classes from previous iterations are collapsed into the background. In this paper, we propose Local POD, a multi-scale pooling distillation scheme that preserves long- and short-range spatial relationships at feature level. Furthermore, we design an entropy-based pseudo-labelling of the background w.r.t. classes predicted by the old model to deal with background shift and avoid catastrophic forgetting of the old classes. Finally, we introduce a novel rehearsal method that is particularly suited for segmentation. Our approach, called PLOP, significantly outperforms state-of-the-art methods in existing CSS scenarios, as well as in newly proposed challenging benchmarks.

==> algo/localpod.tex <==
\begin{algorithm}
\caption{Local POD algorithm}
\label{algo:local_pod}
\begin{algorithmic}[1]
  \Function{Distillation}{$f^t$, $f^{t-1}$, $x$, $S$}
    \State $loss \gets 0$
    \For{\texttt{$l \gets 0$; $l < L$; $l{+}{+}$}}
      \State $\vh^t_l \gets f^t_l(\vx)$
      \State $\vh^{t-1}_l \gets f^{t-1}_l(\vx)$
      
      \State $loss \gets loss + \operatorname{LocalPOD}(\vh^t_l, \vh^{t-1}_l, S)$
    \EndFor
    \State \Return $\frac{loss}{L}$
  \EndFunction
  \\
  \Function{LocalPOD}{$\vh^t$, $\vh^{t-1}, S$} 
    \State $\mathbf{P}^t \gets [\,]$
    \State $\mathbf{P}^{t-1} \gets [\,]$
    
    \For{\texttt{$s \gets 0$; $s < S$; $s{+}{+}$}} \Comment{Eq. 3}
        \State $w \gets \nicefrac{W}{2^s}$
        \State $h \gets \nicefrac{H}{2^s}$

        \For{\texttt{$i \gets 0$; $i < W - w$; $i{+}=w$}}
            \For{\texttt{$j \gets 0$; $j < H - h$; $j{+}=h$}}
                \State $\vp^t \gets \operatorname{\Phi}(\vh^t\texttt{[i:i+w, j:j+h]})$ \Comment{Eq. 1}
                \State $\vp^{t-1} \gets \operatorname{\Phi}(\vh^{t-1}\texttt{[i:i+w, j:j+h]})$ 

                \State $\mathbf{P}^t \|= \vp^t$
                \State $\mathbf{P}^{t-1} \|= \vp^{t-1}$
            \EndFor
        \EndFor
    \EndFor
    \State \Return $\left\Vert \mathbf{P}^t - \mathbf{P}^{t-1}\right\Vert^2$ \Comment{Eq. 5}
  \EndFunction
\end{algorithmic}
\end{algorithm}

==> main.tex <==
\input{content/abstract}
\input{content/introduction}
\input{content/related_work}
\input{content/model}
\input{content/experiments}
\input{content/conclusion}

==> tables/ablations.tex <==
\begin{table}[t]
\centering
\caption{Ablations of \ours on the Pascal-VOC 2012 dataset in 15-5 and 15-1. Scores are measured on a validation subset made of 20\% of the training set.}
\label{tab:ablation}
\begin{tabular}{@{}l||cc|cc@{}}
\toprule
 &  \multicolumn{2}{c}{\textbf{15-5} (2 tasks)} & \multicolumn{2}{c}{\textbf{15-1} (6 tasks)}\\
\cmidrule{2-5}
Model & \textit{all} & \textit{avg} & \textit{all} & \textit{avg}\\
\midrule
CE  & 13.85 & 46.91 & \tableindent 3.99 & 19.37 \\
Pseudo & 66.19 & 73.07 & 19.74 & 44.48 \\
Pseudo + Local POD & 70.29 & 75.13 & 50.41 & 64.95 \\
$\nu$Pseudo + Local POD & \textbf{71.43} & \textbf{75.70} & \textbf{52.31} & \textbf{65.71}\\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
\centering
\caption{Ablations of \ours on the Pascal-VOC 2012 dataset in 15-1. Scores are measured on a validation subset.}
\label{tab:ablation}
\begin{tabular}{@{}p{1cm}>{\centering\arraybackslash}p{0.8cm}>{\centering\arraybackslash}p{0.8cm}|cccc@{}}
\toprule
& \multicolumn{2}{c}{\footnotesize{Local POD}} & \multicolumn{4}{c}{\textbf{15-1}}\\
\cmidrule{2-3}
\scriptsize{Classification} & \scriptsize{Backbone} & \scriptsize{Logits} & 1-15 & 16-20 & \textit{all} & \textit{avg}\\
\midrule
CE  & & & \tableindent 4.70 & \tableindent 1.72 & \tableindent 3.99 & 19.37 \\
Pseudo & & & 24.56 & \tableindent 4.33 & 19.74 & 44.48 \\
Pseudo & \OK & & 51.07 & \tableindent7.04 & 40.58 & 56.38\\
Pseudo & & \OK & 27.41 & \tableindent1.90 & 21.34 & 53.31 \\
Pseudo & \OK & \OK & \textbf{63.22} & \tableindent 9.41 & 50.41 & 64.95 \\
$\nu$Pseudo & \OK & \OK & \textbf{63.06} & \textbf{17.92} & \textbf{52.31} & \textbf{65.71}\\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

==> tables/cityscapes_domain.tex <==
\begin{table}[t]
\centering
\caption{Final mIoU for Continual-domain Cityscapes.}
\label{tab:cityscapes_domain}
\begin{tabular}{@{}l|c||c||c@{}}
\toprule
\textbf{Method} & \textbf{11-5} (3 tasks) & \textbf{11-1} (11 tasks) & \textbf{1-1} (21 tasks)\\
\midrule
%EWC \cite{kirkpatrick2017ewc} & 60.62 & 45.24 & 34.22\\
%LWF-MC \cite{rebuffi2017icarl} & 58.90 & 56.92 & 31.24\\
ILT \cite{michieli2019ilt} & 59.14 & 57.75 & 30.11 \\
MiB \cite{cermelli2020modelingthebackground} & 61.51 & 60.02 & 42.15 \\
\ours & \textbf{63.51} & \textbf{62.05} & \textbf{45.24}\\
% Algo &   &   &   &   &   &  &  &   &   &   &  &  \\
%\midrule
%Joint model & 77.40 & 78.00 & 77.40 & --- & 79.10 & 72.60 & 77.40 & --- & 79.10 & 72.60 & 77.40 & ---\\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
\centering
\caption{Cityscapes domain\tbd}
\label{tab:cityscapes}
\begin{tabular}{@{}l|cccc||cccc@{}}
\toprule
& \multicolumn{2}{c}{\textbf{11-5} (3 tasks)} & \multicolumn{2}{c}{\textbf{11-1} (1 tasks)}\\
\textbf{Method} & \textit{all} & \textit{avg} & \textit{all} & \textit{avg}\\
\midrule
ILT \cite{michieli2019ilt} & 59.14 & 59.14 & 57.65 & 57.92\\
MiB \cite{cermelli2020modelingthebackground} & 61.51 & 59.10 & 59.17 & 57.86\\
\ours & 63.51 & 61.61 & 61.73 & 61.51\\
%\ours w/o adaptive & \textbf{76.05}  & \textbf{33.34}  & \textbf{74.02} & \textbf{75.71} & 75.98 & \textbf{48.95} & 69.54 & 74.91 & \textbf{69.74} & 12.56 & 56.12 & 66.57\\
%\,\,- LP + UNKD & \textbf{76.67}  & 27.08  & \textbf{74.30} & \textbf{75.85} & \textbf{78.53}  & 48.37  & \textbf{71.35} & \textbf{75.82} & 68.87 & \textbf{21.37} & \textbf{57.56} & \textbf{68.56}\\
\midrule
\ours vs MiB \\
% Algo &   &   &   &   &   &  &  &   &   &   &  &  \\
%\midrule
%Joint model & 77.40 & 78.00 & 77.40 & --- & 79.10 & 72.60 & 77.40 & --- & 79.10 & 72.60 & 77.40 & ---\\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

==> tables/erasing_color.tex <==
\begin{table*}[t]
\centering
\caption{Erasing color ablation on Pascal-VOC 2012 in Mean IoU (\%). Object Rehearsal with 10 objects per class.}
\vspace*{-0.3cm}
\label{tab:voc_sota}
\begin{tabular}{@{}l|cccc@{}}
\toprule
 & \multicolumn{4}{c}{\textbf{15-1} (6 tasks)}\\
\textbf{Erasing color} & 1-15 & 16-20 & \textit{all} & \textit{avg}\\
\midrule
Noise & 72.32 & 42.19 & 65.15 & 71.80\\
Mean pixel background & 72.39 & 42.26 & 65.22 & 71.79\\
Mean pixel & 72.86 & 42.49 & 65.63 & 71.86\\
Perlin noise & 72.94 & 42.56 & 65.71 & 71.90\\
Black & 73.10 & 43.31 & 66.01 & 71.95\\
Textures KTH \cite{mallikarjuna2006kth-tips} & 71.99 & 44.34 & 65.41 & 72.08\\
Textures KTH grayscale  \cite{mallikarjuna2006kth-tips} & 71.99 & 44.42 & 65.42 & 72.05\\
InstaBoost's InPainting \cite{fang2019instaboost} & 74.15 & 42.53 & 66.62 & 72.23\\
Half 256/2 = 128 & \textbf{73.79} & \textbf{45.78} & \textbf{67.12} & \textbf{72.42}\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/pseudo_ablations.tex <==
\begin{table}[t]
\centering
\caption{Ablations of the different pseudo-labeling methods evaluated on the Pascal-VOC 2012 dataset in 15-1 overlapped. Scores are measured on a validation subset made of 20\% of the training set.}
\label{tab:ablation}
\begin{tabular}{@{}l||cccc@{}}
\toprule
Pseudo-labeling & \textit{1-15} & \textit{16-20} & \textit{all} & \textit{avg}\\
\midrule
Naive & 68.28 & 10.79 & 54.59 & 66.77\\
Threshold 0.90 & 56.63 & 10.65 & 54.06 & 66.43\\
Median & 66.28 & 11.25 & 53.18 & 65.91\\
Entropy \cite{saporta2020esl} & 63.06 & 17.92 & 52.31 & 65.71\\
\bottomrule
\end{tabular}
\end{table}


==> tables/voc_19-1.tex <==
\begin{table}[t]
\centering
\caption{Continual Semantic Segmentation results on Pascal-VOC 2012 in Mean IoU (\%) on 19-1 overlap setting.}
\vspace*{-0.3cm}
\label{tab:voc_sota}
\begin{tabular}{@{}l|cccc@{}}
\toprule
& \multicolumn{4}{c}{\textbf{19-1} (2 tasks)}\\
\textbf{Method} & 0-19 & 20 & \textit{all} & \textit{avg}\\
\midrule
\text{EWC} \cite{kirkpatrick2017ewc} & 26.90 & 14.00 & 26.30 &   \\
\text{LwF-MC} \cite{rebuffi2017icarl} & 64.40 & 13.30 & 61.90 &  \\
%$\text{ILT}^\dagger$ \cite{michieli2019ilt} & 67.10 & 12.30 & 64.40 &  & 66.30 & 40.60 & 59.90 &  \\ 
$\text{ILT}$ \cite{michieli2019ilt} & 67.75 & 10.88 & 65.05 & 71.23 \\ 
%$\text{MiB}^\dagger$ \cite{cermelli2020modelingthebackground} & 70.20 & 22.10 & 67.80 &    & 75.50 & 49.40 & 69.00 &  & 35.10 & 13.50 & 29.70 & \\
MiB \cite{cermelli2020modelingthebackground} & 71.43 & 23.59 & 69.15  & 73.28 \\
\ours & \textbf{75.35} & \textbf{37.35} & \textbf{73.54} & \textbf{75.47}\\
\bottomrule
\end{tabular}
\end{table}


==> tables/voc_disjoint.tex <==
\begin{table*}[t]
\centering
\caption{Mean IoU on the Pascal-VOC 2012 dataset for different incremental class learning scenarios, all in Disjoint. $\dagger$ denotes results from Cermelli et al.\cite{cermelli2020modelingthebackground}.}
\label{tab:voc_disjoint_sota}
\begin{tabular}{@{}l|cccc||cccc||cccc@{}}
\toprule
& \multicolumn{4}{c}{\textbf{19-1} (2 tasks)} & \multicolumn{4}{c}{\textbf{15-5} (2 tasks)} & \multicolumn{4}{c}{\textbf{15-1} (6 tasks)}\\
\textbf{Method} & 0-19 & 20 & \textit{all} & \textit{avg} & 0-15 & 16-20 & \textit{all} & \textit{avg} & 0-15 & 16-20 & \textit{all} & \textit{avg}\\
\midrule
% from paper MiB
$\text{Fine Tuning}^\dagger$ & \tableindent 5.80 & 12.30 & \tableindent 6.20 & & \tableindent 1.10 & 33.60 & \tableindent 9.20 & & \tableindent 0.20 & \tableindent 1.80 & \tableindent 0.60 \\
$\text{PI}^\dagger$ \cite{zenke2017synaptic_intelligence} & \tableindent 5.40 & 14.10 & \tableindent 5.90 & & \tableindent 1.30 & 34.10 & \tableindent 9.50 & & \tableindent 0.00 & \tableindent 1.80 & \tableindent 0.40 & \\
$\text{EWC}^\dagger$ \cite{kirkpatrick2017ewc} & 23.20 & 16.00 & 22.90 & & 26.70 & 37.70 & 29.40 & & \tableindent 0.30 & \tableindent 4.30 & \tableindent 1.30 & \\
$\text{RW}^\dagger$ \cite{chaudhry2018riemannien_walk} & 19.40 & 15.70 & 19.20 & & 17.90 & 36.90 & 22.70 & & \tableindent 0.20 & \tableindent 5.40 & \tableindent 1.50 & \\
$\text{LwF}^\dagger$ \cite{li2018lwf} & 53.00 & \tableindent 9.10 & 50.80 & & 58.40 & 37.40 & 53.10 & & \tableindent 0.80 & \tableindent 3.60 & \tableindent 1.50 & \\
$\text{LwF-MC}^\dagger$ \cite{rebuffi2017icarl} & 63.00 & 13.20 & 60.50 & & 67.20 & 41.20 & 60.70 & & \tableindent 4.50 & \tableindent 7.00 & \tableindent 5.20 & \\
$\text{ILT}^\dagger$ \cite{michieli2019ilt} & 69.10 & 16.40 & 66.40 & & 63.20 & 39.50 & 57.30 & & \tableindent 3.70 & \tableindent 5.70 & \tableindent 4.20 &  \\ 
%$\text{ILT}$ \cite{michieli2019ilt} & 71.17 & 16.12 & 68.55 & 73.59 & 64.92 & 38.75 & 58.69 & 69.15 & 10.17 & \tableindent 8.31 & \tableindent 9.73 & 41.05\\ 

$\text{MiB}^\dagger$ \cite{cermelli2020modelingthebackground} & 69.60 & 25.60 & 67.40 & & \textbf{71.80} & \textbf{43.30} & \textbf{64.70} & & 46.20 & 12.90 & 37.90 & \\
% from us
%MiB \cite{cermelli2020modelingthebackground} & 71.22 & 20.95 & 68.83 & 73.60 & \textbf{73.68} & \textbf{45.32} & \textbf{66.93} & \textbf{72.99} & 40.99 & 12.68 & 34.25 & 58.09\\

\ours & \textbf{75.37} & \textbf{38.89} & \textbf{73.64} & 75.71 & \textbf{71.00} & \textbf{42.82} & \textbf{64.29} & 72.05 & \textbf{57.86} & \textbf{13.67} & \textbf{46.48} & 62.67\\
%\midrule
%\ours vs MiB &   &   &   &   &   &  &  &   &   &   &  &\\
% Algo &   &   &   &   &   &  &  &   &   &   &  &  \\
%\midrule
%Joint model & 77.40 & 78.00 & 77.40 & --- & 79.10 & 72.60 & 77.40 & --- & 79.10 & 72.60 & 77.40 & ---\\
\bottomrule
\end{tabular}
\end{table*}


==> tables/voc_full.tex <==
\begin{table*}[t]
\centering
\caption{Mean IoU on the Pascal-VOC 2012 dataset for different incremental class learning scenarios, all in Overlap. $\dagger$ denotes results from Cermelli et al.~\cite{cermelli2020modelingthebackground}, all other results are from us.}
\label{tab:voc_sota_full}
\begin{tabular}{@{}l|cccc||cccc||cccc@{}}
\toprule
& \multicolumn{4}{c}{\textbf{19-1} (2 tasks)} & \multicolumn{4}{c}{\textbf{15-5} (2 tasks)} & \multicolumn{4}{c}{\textbf{15-1} (6 tasks)}\\
\textbf{Method} & 0-19 & 20 & \textit{all} & \textit{avg} & 0-15 & 16-20 & \textit{all} & \textit{avg} & 0-15 & 16-20 & \textit{all} & \textit{avg}\\
\midrule
% from paper MiB
$\text{Fine Tuning}^\dagger$ & \tableindent 6.80 & 12.90 & \tableindent 7.10 &  & \tableindent 2.10 & 33.10 & \tableindent 9.80 &  & \tableindent 0.20 & \tableindent 1.80 & \tableindent 0.60 & \\
$\text{PI}^\dagger$ \cite{zenke2017synaptic_intelligence} & \tableindent 7.50 & 14.00 & \tableindent 7.80 &  & \tableindent 1.60 & 33.30 & \tableindent 9.50 &  & \tableindent 0.00 & \tableindent 1.80 & \tableindent 0.50 & \\
$\text{EWC}^\dagger$ \cite{kirkpatrick2017ewc} & 26.90 & 14.00 & 26.30 &  & 24.30 & 35.50 & 27.10 &  & \tableindent 0.30 & \tableindent 4.30 & \tableindent 1.30 &  \\
$\text{RW}^\dagger$ \cite{chaudhry2018riemannien_walk} & 23.30 & 14.20 & 22.90 &  & 16.60 & 34.90 & 21.20 &  & \tableindent 0.00 & \tableindent 5.20 & \tableindent 1.30 & \\
$\text{LwF}^\dagger$ \cite{li2018lwf} & 51.20 & \tableindent 8.50 & 49.10 &  & 58.90 & 36.60 & 53.30 &  & \tableindent 1.00 & \tableindent 3.90 & \tableindent 1.80 & \\
$\text{LwF-MC}^\dagger$ \cite{rebuffi2017icarl} & 64.40 & 13.30 & 61.90 &  & 58.10 & 35.00 & 52.30 &  & \tableindent 6.40 & \tableindent 8.40 & \tableindent 6.90 & \\
$\text{ILT}^\dagger$ \cite{michieli2019ilt} & 67.10 & 12.30 & 64.40 &  & 66.30 & 40.60 & 59.90 &  & \tableindent 4.90 & \tableindent 7.80 & \tableindent 5.70 & \\ 
$\text{ILT}$ \cite{michieli2019ilt} & 67.75 & 10.88 & 65.05 & 71.23 & 67.08 & 39.23 & 60.45 & 70.37 & \tableindent 8.75 & \tableindent 7.99 & \tableindent 8.56 & 40.16 \\ 

$\text{MiB}^\dagger$ \cite{cermelli2020modelingthebackground} & 70.20 & 22.10 & 67.80 &    & 75.50 & 49.40 & 69.00 &  & 35.10 & 13.50 & 29.70 & \\
% from us
MiB \cite{cermelli2020modelingthebackground} & 71.43 & 23.59 & 69.15  & 73.28  & \textbf{76.37}  & 49.97  & \textbf{70.08} & \textbf{75.12} & 34.22 & 13.50  & 29.29  & 54.19 \\

\ours & \textbf{75.35} & \textbf{37.35} & \textbf{73.54} & \textbf{75.47} & 75.73 & \textbf{51.71} & \textbf{70.09} & \textbf{75.19} & \textbf{65.12} & \textbf{21.11} & \textbf{54.64} & \textbf{67.21}\\
%\midrule
%\ours vs MiB & +3.92 & +13.76 & +4.39 & +1.19 & -0.64 & +1.84 & +0.01 & +0.07 & +30.90 & +7.61 & +25.35 & +13.02\\
% Algo &   &   &   &   &   &  &  &   &   &   &  &  \\
%\midrule
%Joint model & 77.40 & 78.00 & 77.40 & --- & 79.10 & 72.60 & 77.40 & --- & 79.10 & 72.60 & 77.40 & ---\\
\bottomrule
\end{tabular}
\end{table*}

